Rapidity distribution of pseudo-scalar Higgs boson to $\rm{\textbf{NNLO}_A+\overline{\textbf {NNLL}}}$

We present the differential predictions for the rapidity distribution of pseudo-scalar Higgs boson through gluon fusion at the LHC. These results are obtained taking into account the soft-virtual (SV) as well as the next-to-soft virtual (NSV) resummation effects to next-to-next-to-leading-logarithmic ($\rm{\overline{NNLL}}$) accuracy and matching them to the approximate fixed order next-to-next-to-leading-order ($\rm{NNLO_A}$) computation. We perform the resummation in two dimensional Mellin space using our recent formalism \cite{Ajjath:2020lwb} by limiting ourselves to the contributions only from gluon-gluon ($gg$) initiated channels. The $\rm{NNLO_A}$ rapidity distribution of pseudo-scalar Higgs is obtained by applying a ratio method on the NNLO rapidity distribution of the scalar Higgs boson. We also present the first analytical results of $\rm{N^3LO}$ rapidity distribution of pseudo-scalar Higgs at SV+NSV accuracy. The phenomenological impacts of $\rm{{NNLO}_A+\overline{{NNLL}}}$ predictions for 13 TeV LHC are studied. We observe that, for $m_A$ =125(700) GeV, the SV+NSV resummation at $\rm{ \overline{NNLL}}$ level brings about 14.76\% (11.48\%) corrections to the $\rm{NNLO}_A$ results at the central scale value of $\mu_R=\mu_F=m_A$. Further, we find that the sensitivity to the renormalisation scale gets improved substantially by the inclusion of NSV resummed predictions at $\rm \overline{NNLL}$ accuracy.

==> NSVH.tex <==
\begin{align}
\begin{autobreak}

\Delta_{d,g}^{H,\rm NSV} = 

a_s \Delta_{d,g}^{\rm NSV,(1)} + a_s^2 \Delta_{d,g}^{\rm NSV,(2)} + a_s^3 \Delta_{d,g}^{\rm NSV,(3)} +

        {\color{blue} \pmb{a_s^4}} \Bigg\{ 
             C_A^4   \bigg[
            {\color{black}{L^{7}_{z_1}}} \Big( 
          - \frac{16}{3}  \bar {\delta} \Big)
          + {\color{black}{L^{6}_{z_1}}} \Big(
          
          - \frac{112}{3} \overline{\cal D}_0
           + \frac{692}{9} \bar {\delta} \Big) 
          + {\color{black}{L^{5}_{z_1}}} \Big( 
            \frac{1336}{3}  \overline{\cal D}_0
          
          - 224 \overline{\cal D}_1  +
          \bar {\delta} \Big( 144 \zeta_2 - \frac{12224}{27} \Big)
          \Big)
          \bigg]
          
  +        C_A^3 n_f    \bigg[
          {\color{black}{L^{6}_{z_1}}} \Big(
        -  \frac{56}{9} \bar {\delta} \Big) 
        + {\color{black}{L^{5}_{z_1}}} \Big( 
         
        - \frac{112}{3}  \overline{\cal D}_0 
        +  \frac{796}{9}  \bar {\delta}\Big)
          \bigg]
          
         +          C_A^2 n_f^2 \bigg[{\color{black}{L^{5}_{z_1}}} \Big(  - \frac{64}{27}  \bar {\delta} \Big) \bigg] + \mathcal{O}\Big( {\color{black}{ L^4_{z_1}}} \Big) \Bigg\}
          
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        + {\color{blue} \pmb{a_s^5}} \Bigg\{
         C_A^5  \bigg[ L_{z_1}^9   \Big(
          - \frac{8}{3} \bar{\delta}
          \Big)

       + L_{z_1}^8   \Big(
          - 24 {\cal D}_0
          + \frac{172}{3} \bar{\delta}
          \Big)

       +  L_{z_1}^7   \Big(
            448 {\cal D}_0
          - 192 {\cal D}_1
          - \bar{\delta} \Big( \frac{42536}{81} 
          - \frac{448}{3} \zeta_2 
          \Big) \Big) \bigg]

   

       + C_A^4 n_f  \bigg[ L_{z_1}^8   \Big(
          - \frac{16}{3} \bar{\delta}
          \Big)

       +  L_{z_1}^7   \Big(
          - \frac{128}{3} {\cal D}_0
          + \frac{9016}{81} \bar{\delta}
          \Big) \bigg]

   

       + C_A^3 n_f^2 \bigg[ L_{z_1}^7    \Big(- \frac{320}{81} \bar{\delta}\Big)  \bigg] + \mathcal{O}\Big( {\color{black}{ L^6_{z_1}}} \Big) \Bigg\} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

        + {\color{blue} \pmb{a_s^6}} \Bigg\{

        C_A^6 \bigg[ L_{z_1}^{11}   \Big(
          - \frac{16}{15} \bar{\delta}
          \Big)

       + L_{z_1}^{10}   \Big(
          - \frac{176}{15} {\cal D}_0
          + \frac{4292}{135} \bar{\delta}
          \Big)

       +  L_{z_1}^9   \Big(
            \frac{8440}{27} {\cal D}_0
          - \frac{352}{3} {\cal D}_1
          - \bar{\delta} \Big( \frac{33568}{81} 
          - \frac{304}{3} \zeta_2  \Big)
          \Big) \bigg]

   

       + C_A^5 n_f  \bigg[ L_{z_1}^{10}   \Big(
          - \frac{88}{27} \bar{\delta}
          \Big)

       +  L_{z_1}^9   \Big(
          - \frac{880}{27} {\cal D}_0
          + \frac{2524}{27} \bar{\delta}
          \Big) \bigg]

   

       + C_A^4 n_f^2  \bigg[ L_{z_1}^9   \Big(- \frac{320}{81} \bar{\delta}\Big) \bigg] + \mathcal{O}\Big( {\color{black}{ L^8_{z_1}}} \Big) \Bigg\}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
       + {\color{blue} \pmb{a_s^7}} \Bigg\{
        C_A^7 \bigg[ L_{z_1}^{13}   \Big(
          - \frac{16}{45} \bar{\delta}
          \Big)

       + L_{z_1}^{12}   \Big(
          - \frac{208}{45} {\cal D}_0
          + \frac{1888}{135} \bar{\delta}
          \Big)

       +   L_{z_1}^{11}   \Big(
          \frac{7456}{45} {\cal D}_0
          - \frac{832}{15} {\cal D}_1
          - \bar{\delta} \Big( \frac{11024}{45} 
          + \frac{256}{5} \zeta_2  \Big)
          \Big) \bigg]

   

       + C_A^6 n_f  \bigg[L_{z_1}^{12}   \Big(
          - \frac{208}{135} \bar{\delta}
          \Big)

       +  L_{z_1}^{11}   \Big(
          - \frac{832}{45} {\cal D}_0
          + \frac{23512}{405} \bar{\delta}
          \Big) \bigg]

        + C_A^5 n_f^2 \bigg[ L_{z_1}^{11}   \Big(- \frac{224}{81} \bar{\delta} \Big) \bigg] + \mathcal{O}\Big( {\color{black}{ L^{10}_{z_1}}} \Big) \Bigg\}  +  \big( z_1 \leftrightarrow z_2 \big)\,.

\end{autobreak}
\end{align}


==> lnGamma.tex <==
\begin{align}
    
\ln \Gamma_{gg}^P(z_j, \mu_F^2) &=
  a_s(\mu_F^2) \bigg\{ \delta(\bar z_j)
       \bigg[ \frac{1}{\epsilon} n_f   \bigg(  - \frac{4}{3} \bigg)

       + \frac{1}{\epsilon} C_A   \bigg( \frac{22}{3} \bigg) \bigg]

     + {\cal D}_0(z_j)
       \bigg[  \frac{1}{\epsilon} 8 C_A    \bigg]

  
       -  \frac{1}{\epsilon} 8 C_A  \bigg\}

\nonumber\\&
 + a_s(\mu_F^2)^2 \bigg\{ \delta(\bar z_j)
       \bigg[ \frac{1}{\epsilon^2} n_f^2   \bigg( \frac{8}{9} \bigg)

       + \frac{1}{\epsilon^2} C_A n_f   \bigg(  - \frac{88}{9} \bigg)

       + \frac{1}{\epsilon^2} C_A^2   \bigg( \frac{242}{9} \bigg)

       - \frac{1}{\epsilon} 2 C_F n_f   
\nonumber\\&
       + \frac{1}{\epsilon} C_A n_f   \bigg(  - \frac{8}{3} \bigg)

       + \frac{1}{\epsilon} C_A^2   \bigg( \frac{32}{3} + 12 \zeta_3 \bigg) \bigg]

  +  {\cal D}_0(z_j)
       \bigg[ \frac{1}{\epsilon^2} C_A n_f   \bigg(  - \frac{16}{3} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^2} C_A^2   \bigg( \frac{88}{3} \bigg)

       + \frac{1}{\epsilon} C_A n_f   \bigg(  - \frac{40}{9} \bigg)

       + \frac{1}{\epsilon} C_A^2   \bigg( \frac{268}{9} - 8 \zeta_2 \bigg) \bigg]

 + L(z_j)
       \bigg[ \frac{1}{\epsilon} 16 C_A^2  \bigg]
  \nonumber\\&     
      +  \frac{1}{\epsilon^2} C_A n_f   \bigg( \frac{16}{3} \bigg)
    
       + \frac{1}{\epsilon^2} C_A^2   \bigg(  - \frac{88}{3} \bigg)

       + \frac{1}{\epsilon} C_A n_f   \bigg( \frac{40}{9} \bigg)

       + \frac{1}{\epsilon} C_A^2   \bigg(  - \frac{268}{9} + 8 \zeta_2 \bigg)

 \bigg\} 
   \nonumber\\& 
  + a_s(\mu_F^2)^3 \bigg\{ \delta(\bar z_j) 
       \bigg[ \frac{1}{\epsilon^3} n_f^3   \bigg(  - \frac{64}{81} \bigg)
     
       + \frac{1}{\epsilon^3} C_A n_f^2   \bigg( \frac{352}{27} \bigg)

       + \frac{1}{\epsilon^3} C_A^2 n_f   \bigg(  - \frac{1936}{27} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^3} C_A^3   \bigg( \frac{10648}{81} \bigg)

       + \frac{1}{\epsilon^2} C_F n_f^2   \bigg( \frac{32}{9} \bigg)
     
       + \frac{1}{\epsilon^2} C_A n_f^2   \bigg( \frac{16}{3} \bigg)

       + \frac{1}{\epsilon^2} C_A C_F n_f   \bigg(  - \frac{176}{9} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^2} C_A^2 n_f   \bigg(  - \frac{440}{9} - \frac{32}{3} \zeta_3 \bigg)

       + \frac{1}{\epsilon^2} C_A^3   \bigg( \frac{968}{9}  + \frac{176}{3} \zeta_3 \bigg)

       + \frac{1}{\epsilon} C_F n_f^2   \bigg( \frac{22}{27} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon} C_F^2 n_f   \bigg( \frac{2}{3} \bigg)

       + \frac{1}{\epsilon} C_A n_f^2   \bigg( \frac{29}{27} \bigg)

       + \frac{1}{\epsilon} C_A C_F n_f   \bigg(  - \frac{241}{27} \bigg)

       + \frac{1}{\epsilon} C_A^2 n_f   \bigg(  - \frac{233}{27}
       \nonumber\\&
       - \frac{160}{9} \zeta_3 - \frac{16}{9} \zeta_2 - \frac{8}{9} \zeta_2^2
          \bigg)

       + \frac{1}{\epsilon} C_A^3   \bigg( \frac{79}{3} 
       - \frac{160}{3} \zeta_5 + \frac{1072}{9} \zeta_3 + \frac{16}{9} \zeta_2 - \frac{32}{3}
          \zeta_2 \zeta_3 
          \nonumber\\&
          + \frac{44}{9} \zeta_2^2 \bigg) \bigg]

    + {\cal D}_0(z_j)
       \bigg[ \frac{1}{\epsilon^3} C_A n_f^2   \bigg( \frac{128}{27} \bigg)

       + \frac{1}{\epsilon^3} C_A^2 n_f   \bigg(  - \frac{1408}{27} \bigg)

       + \frac{1}{\epsilon^3} C_A^3   \bigg( \frac{3872}{27} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^2} C_A n_f^2   \bigg( \frac{320}{81} \bigg)

       + \frac{1}{\epsilon^2} C_A C_F n_f   \bigg(  - \frac{32}{3} \bigg)

       + \frac{1}{\epsilon^2} C_A^2 n_f   \bigg(  - \frac{5344}{81} + \frac{64}{9} \zeta_2 \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^2} C_A^3   \bigg( \frac{16688}{81} - \frac{352}{9} \zeta_2 \bigg)

       + \frac{1}{\epsilon} C_A n_f^2   \bigg(  - \frac{32}{81} \bigg)

       + \frac{1}{\epsilon} C_A C_F n_f   \bigg(  - \frac{220}{9} + \frac{64}{3} \zeta_3 \bigg)
\nonumber\\&
       + \frac{1}{\epsilon} C_A^2 n_f   \bigg(  - \frac{1672}{81} - \frac{224}{9} \zeta_3 + \frac{320}{27} \zeta_2 \bigg)

       + \frac{1}{\epsilon} C_A^3   \bigg( \frac{980}{9} + \frac{176}{9} \zeta_3 - \frac{2144}{27} \zeta_2 
       \nonumber\\&
       + \frac{352}{15} \zeta_2^2
          \bigg) \bigg]

     +  L(z_j)
       \bigg[ \frac{1}{\epsilon^2} C_A^2 n_f   \bigg(  - \frac{128}{9} \bigg)

       + \frac{1}{\epsilon^2} C_A^3   \bigg( \frac{704}{9} \bigg)

       + \frac{1}{\epsilon} C_A^2 n_f   \bigg(  - \frac{640}{27} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon} C_A^3   \bigg( \frac{4288}{27}
  
       - \frac{128}{3} \zeta_2 \bigg) \bigg]

     +   \frac{1}{\epsilon^3} C_A n_f^2   \bigg(  - \frac{128}{27} \bigg)

       + \frac{1}{\epsilon^3} C_A^2 n_f   \bigg( \frac{1408}{27} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^3} C_A^3   \bigg(  - \frac{3872}{27} \bigg)

       + \frac{1}{\epsilon^2} C_A n_f^2   \bigg(  - \frac{320}{81} \bigg)

       + \frac{1}{\epsilon^2} C_A C_F n_f   \bigg( \frac{32}{3} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon^2} C_A^2 n_f   \bigg( \frac{5344}{81} - \frac{64}{9} \zeta_2 \bigg)

       + \frac{1}{\epsilon^2} C_A^3   \bigg(  - \frac{16688}{81} + \frac{352}{9} \zeta_2 \bigg)

       + \frac{1}{\epsilon} C_A n_f^2   \bigg( \frac{32}{81} \bigg)
\nonumber\\&
       + \frac{1}{\epsilon} C_A C_F n_f   \bigg( \frac{220}{9} - \frac{64}{3} \zeta_3 \bigg)

       + \frac{1}{\epsilon} C_A^2 n_f   \bigg( \frac{1816}{81} + \frac{224}{9} \zeta_3 - \frac{320}{27} \zeta_2 \bigg)
\nonumber\\&
       + \frac{1}{\epsilon} C_A^3   \bigg(  - \frac{332}{3} + \frac{112}{9} \zeta_3 + \frac{2144}{27} \zeta_2 - \frac{352}{15} 
         \zeta_2^2 \bigg) \bigg\}\,.
\end{align}


==> phirel.tex <==

The generic expressions for the NSV coefficient $\varphi^{A,(i,k)}_{d,g}$ in terms of NSV inclusive counterpart coefficient $\varphi^{A,(i,k)}_g$ and anomalous dimensions like cusp $A^A_g$, collinear $B^A_g$, soft $f^A_g$ and $C^A_g$ and $D^A_g$ from NSV part of splitting function, are given below,
\begin{align}
\label{eq:Phirel}
\varphi^{c,(0)}_{d,1} &=  
            C^{c}_1 \zeta_2 + \varphi^{(0)}_{c,1} - \frac{1}{2} A^c_1 \,,
\nonumber \\  
\varphi^{c,(0)}_{d,2} &=
        \varphi^{(0)}_{c,2}
      - \frac{1}{2} A^c_2
      - \frac{1}{2} \beta_0 f^c_1
      + \zeta_2 C^{c}_2
      - \zeta_2 \beta_0 D^{c}_1 
      + 3 C^{c}_1 \beta_0 \zeta_3
      - \varphi^{(1)}_{c,1} \zeta_2 \beta_0\,,
\nonumber \\  
\varphi^{c,(1)}_{d,2} &= \varphi^{(1)}_{c,2}
      - C^{c}_1 \zeta_2 \beta_0 
\nonumber \\  
\varphi^{c,(0)}_{d,3} &=
        \varphi^{(0)}_{c,3}
      - \frac{1}{2} A^c_3
      - \frac{1}{2} \beta_1 f^c_1
      - \beta_0 f^c_2
      + 6 \beta_0 C^{c}_2 \zeta_3
      - 2 \beta_0^2 \overline{\cal G}^{c,(1)}_{S,1}
      - 4 \beta_0^2 D^{c}_1 \zeta_3
      + 4 \varphi^{(2)}_{c,2} \beta_0 \zeta_3
     + \zeta_2 C^{c}_3 \nonumber \\&  
      - \zeta_2 D^{c}_1 \beta_1
      - 2 \zeta_2 \beta_0 D^{c}_2 
      - 2 \zeta_2 \varphi^{(1)}_{c,2} \beta_0
      + 3 C^{c}_1 \zeta_3 \beta_1
      + \frac{38}{5} C^{c}_1 \zeta_2^2 \beta_0^2
      + 2 \varphi^{(0)}_{c,1} \zeta_2 \beta_0^2
      - A^c_1 \zeta_2 \beta_0^2  \nonumber \\& 
      - 6 \varphi^{(1)}_{c,1} \beta_0^2 \zeta_3
     - \varphi^{(1)}_{c,1} \zeta_2 \beta_1\,,
\nonumber \\  
\varphi^{c,(1)}_{d,3} &=
        \varphi^{(1)}_{c,3}
      - 2 \zeta_2 \beta_0 C^{c}_2
      - 4 \zeta_2 \varphi^{(2)}_{c,2} \beta_0
      - 4 C^{c}_1 \beta_0^2 \zeta_3
      - C^{c}_1 \zeta_2 \beta_1
      + 2 \varphi^{(1)}_{c,1} \zeta_2 \beta_0^2\,.    
\end{align}
